Study of Open Charm Production in p+p Collisions at $\sqrt(s)$ = 200 GeV

The dissertation presents the measurement of electrons from heavy flavor decays in proton + proton collisions at RHIC at collision energy $\sqrt(s) = 200$ GeV. Two independent analysis techniques of signal extraction were performed. This is the first measurement of the Open Charm crossection at this collision energy and it is an important baseline measurement for comparison with nucleus + nucleus collisions. The modification of Open Charm production in heavy ion collisions compared to the presented p+p result can be used to study the final state interaction of the heavy quarks with hot dense matter inside the collisions. The results of the Open Charm measurements are compared to current pQCD predictions both in Leading Order (LO) $O(\alpha_s^2)$ and Next-to-Leading Order (NLO) $O(\alpha_s^3)$. The final result for the total Open Charm crossection is $\sigma_{c\bar{c}}= (0.920 \pm 0.148(stat)\pm 0.524(sys))$ mb.

==> 4/combined_inclusive.tex <==
\begin{table}
\caption{ Initial inclusive invariant crossection.}
\begin{center}
\begin{tabular}[b]{|c|c|c|c|c|c|c|}
\hline $p_{T}$ bin & MB sample &MB sample& ERT sample&ERT sample&Combined&Combined\\
$[GeV/c]$ & crossection&stat. error&crossection&stat. error&crossection&stat. error\\ \hline
0.4-0.5 &8.010e-02 &3.731e-03 &8.323e-02 &1.961e-01 &8.010e-02 &3.731e-03 \\
0.5-0.6 &3.427e-02 &2.113e-03 &2.701e-02 &4.647e-02 &3.426e-02 &2.110e-03 \\
0.6-0.8 &1.308e-02 &8.046e-04 &1.065e-02 &1.124e-02 &1.307e-02 &8.025e-04 \\
0.8-1.0 &3.637e-03 &3.629e-04 &3.803e-03 &2.111e-03 &3.642e-03 &3.576e-04 \\
1.0-1.2 &1.257e-03 &1.899e-04 &1.354e-03 &4.120e-04 &1.274e-03 &1.725e-04 \\
1.2-1.4 &4.487e-04 &1.042e-04 &4.977e-04 &9.092e-05 &4.765e-04 &6.850e-05 \\
1.4-1.6 &2.454e-04 &7.141e-05 &2.626e-04 &3.328e-05 &2.595e-04 &3.017e-05 \\
1.6-2.0 &9.083e-05 &2.893e-05 &8.961e-05 &8.400e-06 &8.971e-05 &8.066e-06 \\
2.0-2.5 &4.028e-05 &1.530e-05 &2.515e-05 &2.594e-06 &2.557e-05 &2.558e-06 \\
2.5-3.0 &1.933e-05 &9.684e-06 &5.052e-06 &9.470e-07 &5.187e-06 &9.425e-07 \\
3.0-4.0 &0.000e+00 &1.127e+08 &1.417e-06 &3.135e-07 &1.417e-06 &3.135e-07 \\
4.0-5.0 &0.000e+00 &1.127e+08 &2.645e-07 &1.189e-07 &2.645e-07 &1.189e-07 \\
\hline \end{tabular} \label{tab:comb_incl} \end{center} \end{table}


==> 4/final_inclusive.tex <==
\begin{table}
\caption{ Final inclusive invariant crossection.}
\begin{center}
\begin{tabular}[b]{|c|c|c|c||}
\hline $p_{T}$ bin & Uncorrected &Final& Final& Correction\\
$[GeV/c]$ & crossection&crossection&stat. error&factor\\ \hline
8.010e-02 &7.742e-02 &3.606e-03 &0.967\\
3.426e-02 &3.334e-02 &2.054e-03 &0.973\\
1.307e-02 &1.204e-02 &7.398e-04 &0.922\\
3.642e-03 &3.435e-03 &3.374e-04 &0.943\\
1.274e-03 &1.219e-03 &1.650e-04 &0.957\\
4.765e-04 &4.605e-04 &6.619e-05 &0.966\\
2.595e-04 &2.525e-04 &2.935e-05 &0.973\\
8.971e-05 &8.266e-05 &7.433e-06 &0.921\\
2.557e-05 &2.342e-05 &2.342e-06 &0.916\\
5.187e-06 &4.873e-06 &8.854e-07 &0.939\\
1.417e-06 &1.204e-06 &2.664e-07 &0.850\\
2.645e-07 &2.386e-07 &1.072e-07 &0.902\\
\hline \end{tabular} \label{tab:final_incl} \end{center} \end{table}


==> 4/final_subtracted.tex <==
\begin{table}
\caption{ Non-photonic electron invariant crossection.}
\begin{center}
\begin{tabular}[b]{|c|c|c|c|}
\hline $p_{T}$ bin & Non-photonic & Non-photonic & Relative\\
$[GeV/c]$ & crossection&stat. error&error [\%]\\
& $\cunit$ &$\cunit$&\\ \hline
0.4-0.5 &1.454e-02 &3.323e-03 &22.9 \\
0.5-0.6 &6.118e-03 &1.920e-03 &31.4 \\
0.6-0.8 &2.967e-03 &7.154e-04 &24.1 \\
0.8-1.0 &8.427e-04 &3.251e-04 &38.6 \\
1.0-1.2 &3.634e-04 &1.436e-04 &39.5 \\
1.2-1.4 &1.350e-04 &4.813e-05 &35.6 \\
1.4-1.6 &1.133e-04 &2.136e-05 &18.8 \\
1.6-2.0 &3.872e-05 &6.076e-06 &15.7 \\
2.0-2.5 &1.366e-05 &2.213e-06 &16.2 \\
2.5-3.0 &2.577e-06 &8.832e-07 &34.3 \\
3.0-4.0 &8.396e-07 &2.715e-07 &32.3 \\
4.0-5.0 &1.894e-07 &1.086e-07 &57.4 \\
\hline \end{tabular} \label{tab:final_nonphotonic} \end{center} \end{table}


==> 4/initial_inclusive.tex <==
\begin{table}
\caption{ Initial inclusive invariant crossection.}
\begin{center}
\begin{tabular}[b]{|c|c|c|c|c|c|c|}
\hline $p_{T}$ bin & MB sample &MB sample& ERT sample&ERT sample&Random bg&Random bg\\
$[GeV/c]$ & crossection&stat. error&crossection&stat. error&crossection&stat. error\\ \hline
0.4-0.5 &8.295e-02 &3.731e-03 &8.608e-02 &2.629e-02 &2.846e-03 &1.199e-05 \\
0.5-0.6 &3.514e-02 &2.113e-03 &2.788e-02 &4.048e-03 &8.657e-04 &5.766e-06 \\
0.6-0.8 &1.331e-02 &8.046e-04 &1.088e-02 &6.674e-04 &2.309e-04 &1.839e-06 \\
0.8-1.0 &3.692e-03 &3.629e-04 &3.858e-03 &1.432e-04 &5.474e-05 &7.657e-07 \\
1.0-1.2 &1.272e-03 &1.899e-04 &1.369e-03 &5.185e-05 &1.584e-05 &3.684e-07 \\
1.2-1.4 &4.535e-04 &1.042e-04 &5.025e-04 &2.433e-05 &4.802e-06 &1.862e-07 \\
1.4-1.6 &2.472e-04 &7.141e-05 &2.643e-04 &1.529e-05 &1.754e-06 &1.051e-07 \\
1.6-2.0 &9.138e-05 &2.893e-05 &9.017e-05 &5.584e-06 &5.546e-07 &3.889e-08 \\
2.0-2.5 &4.037e-05 &1.530e-05 &2.523e-05 &2.309e-06 &8.292e-08 &1.212e-08 \\
2.5-3.0 &1.936e-05 &9.684e-06 &5.076e-06 &9.285e-07 &2.393e-08 &5.808e-09 \\
3.0-4.0 &0.000e+00 &0.000e+00 &1.420e-06 &3.109e-07 &3.447e-09 &1.412e-09 \\
4.0-5.0 &0.000e+00 &0.000e+00 &2.650e-07 &1.187e-07 &4.796e-10 &4.796e-10 \\
\hline \end{tabular} \label{tab:init_incl} \end{center} \end{table}

